Multiple zeta values in $\lambda$-rings

We propose a framework for multiple zeta values in $\lambda$-rings that unifies both classical multiple zeta values and multiple $q$-zeta values. As in the classical case, we show that the multiple zeta function defines an algebra homomorphism from the quasi-shuffle algebra to the $\lambda$-ring. We also prove a formula for multiple polylogarithms in $\lambda$-rings, similar to the iterated integral expression in the classical case. As an application, we explicitly describe the algebra of regular multiple $q$-zeta values, compute the corresponding Poincar\'e series, and exhibit a small spanning set.

==> commands.tex <==
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{etoolbox,xspace,scalerel}
\RequirePackage{version,xparse}
\RequirePackage[capitalize]{cleveref}
\makeatletter

%%%% Theorem environments
%\ifx\theorem\undefined
\ifundef\theorem{
  \newtheorem{thm}{Theorem}[section]
  \def\newthmx#1#2{
    \ifcsundef{#1}{
      \newtheorem{#1}[thm]{#2}
      \AddToHook{env/#1/begin}{\crefalias{thm}{#1}} %fix cleveref
    }{}
  }
  \def\newthm#1{\newthmx{#1}{\MakeUppercase#1}}

  \theoremstyle{plain}
  \forcsvlist\newthm{theorem,lemma,corollary,proposition,conjecture}
  \theoremstyle{definition}
  \forcsvlist\newthm{definition,remark,example,question,claim,exercise}
  \theoremstyle{remark}
  \newthmx{rmr}{Remark}
}{}

% References
%\numberwithin{equation}{section} %before thmtools, hyperref?

%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}} %define math command
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\opn{\operatorname}
\def\opr#1#2{\dmat#1{\opn{#2}}}
\def\DMO{\opr}
\def\csopr#1#2{\csdmat{#1}{\opn{#2}}}
\def\oper#1{\csopr{#1}{#1}}
\def\operl{\forcsvlist\oper}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\newcommand\envalias[2]{\newenvironment{#1}{\begin{#2}}{\end{#2}}}


%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,Re,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,sgn,Li,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Proj,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,Td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id,Span,Arg,Bl,wt,Cone,
coim,Coim,eq,coeq,Eq,Coeq}

\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lEnd{\lb{End}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\sign{\sgn}
\opr\spn{span}

\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\pt{\mathbf{pt}}
\def\opfrak#1{\csdef{#1}{\mathfrak{#1}}}
\forcsvlist\opfrak{gl,sl,su,so}
\def\oprm#1{\csdef{#1}{\mathrm{#1}}}
\forcsvlist\oprm{op,nil,et,sep,ab,top,tf,}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\def\Vecf{\Vect_{\mathrm f}}

%%%% Arrows
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\RequirePackage{mathtools}
\def\xmto{\xmapsto}
\def\xlto{\xleftarrow}
\def\xemb{\xhookrightarrow}
\def\xonto#1{\xto{#1}\mathrel{\mkern-14mu}\to}
\def\dashto{\dashrightarrow}
\def\dto{\dashrightarrow}
\def\dashlto{\dashlefttarrow}
\def\dlto{\dashlefttarrow}

%%% Symbols
\redef{iff}
\dmat\imp{\implies}
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\ms{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\def\sbe{\subseteq}
\def\spe{\supseteq}
\dmat\xx{\times}
\dmat\Cx{\bC^\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\isoc{\cong} %canonical isomorphism
%\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
%\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\NewDocumentCommand\ubar{O{1.5}O{1.5}m}{%
  \mkern#1mu\overline{\mkern-#1mu#3\mkern-#2mu}\mkern#2mu}

\def\oh{{\frac12}}
\def\toh{{\tfrac12}}
\RequirePackage{bbm}
\dmat\one{\mathbbm1} %requires bbm
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\partof{\vdash}
\def\adj{\mathrel{\tikz
\draw[line cap=round](0,0)--(0,1.5ex)(0,.75ex)--(-1.5ex,.75ex);}}
%\def\adj{\mathrel{\relbar\mkern-14mu\vcenter{\hbox{$\dashv$}}}}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\trp{^{\mathsf T}} %transpose
\dmat\bul{\bullet}
\def\GIT{/\!\!/}
\def\git{\GIT}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\m{\wedge}
\def\j{\vee}
\def\blank{\scalebox{.8}{$-$}} %blank argument

\def\upc{\tikz{\draw[->,>=latex'](0,0)--(0,.3)}}
%requires \usetikzlibrary{arrows}
\def\upc#1{\left\uparrow#1\right.}%upper closure
\def\loc#1{\left\downarrow#1\right.}%lower closure
\def\cupp{\!\smallsmile\!} %cup product
\def\capp{\!\smallfrown\!} %cap product

\def\vcenterx#1{\vcenter{\hbox{#1}}}
\def\rsbox#1#2#3{% raise and scale
  \raisebox{#1}{\scalebox{#2}{\ensuremath{#3}}}}
\NewDocumentCommand\cscale{O{0pt} O{.7} m}{%
  %Central scale: #1-raise, #2-scale, #3-argument
  \ThisStyle{\vcenterx{\rsbox{#1}{#2}{\SavedStyle#3}}}}


\def\isoto{\xto{\,\smash{\rsbox{-3pt}{.8}\sim}\,}}
%\def\dual{^{\cscale[.8]{\vee}}}
\def\dual{^{\scalerel*\vee{*}}}
\def\sbul{\cscale[1pt][.7]{\bullet}}
%\def\ac{{\tiny\raisebox{2pt}{\textup{!}}}}%anti-shriek?
\def\ac{{\scalerel*{\rotatebox[origin=c]{180}{!}}{!}}}

\usepackage[T2A]{fontenc} %T2A, OT2
%\def\sha{\mathord{\textup\cyrsh}}
\DeclareSymbolFont{cyrletters}{T2A}{cmr}{m}{n}
\DeclareMathSymbol{\sha}{\mathbin}{cyrletters}{\cyrsh}

\let\t@sum\sum
\def\sum{\@ifstar{\t@sum\nolimits}\t@sum}
\let\t@prod\prod
\def\prod{\@ifstar{\t@prod\nolimits}\t@prod}
\let\t@bop\bigoplus
\def\bop{\@ifstar{\t@bop\nolimits}\t@bop}
\def\bts{\@ifstar{\bigotimes\nolimits}\bigotimes}

\newcommand\tcd[2][]{%
  \begin{tikzcd}[#1,ampersand replacement=\&]#2\end{tikzcd}}

\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}

\newcommand\edge[2][1.5em]{%\xrightarrow without tip
  \tcd[cramped,column sep=#1]{\rar[-,"#2"]\&{}}}


%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\flist#1#2{\expandafter\forcsvlist\expandafter#1\expandafter{#2}}
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defrm#1{\csdmat{r#1}{\mathrm{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}%
  \defsf{#1}\defrm{#1}}

\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

\def\deflbf#1{\csdmat{b#1}{\mathbf{#1}}} %lower case bf
\forcsvlist\deflbf{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
\forcsvlist\defbf{f,k,m} %\bff,\bfk,\bfm
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}
\defrm{i} %\ri


%%%% Greek letters
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\ep\epsilon
\dmat\io{\iota}
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu,rho}

%%%% Structures
\RequirePackage{mleftright} %better spaces
\def\lr#1#2#3{\mleft#1#2\mright#3}
\def\set#1{\lr\{{#1}\}}
%\def\sets#1#2{\set{#1\,\lr|{\,\vphantom{#1}#2}.}}
\def\sets#1#2{\set{#1\,\middle|\,#2}}
\def\setc#1#2{\set{#1\col#2}}
\def\ang#1{\lr\langle{#1}\rangle}
\def\angs#1#2{\ang{#1\col#2}}
\def\rbr#1{\lr({#1})} %round bracket
\def\sbr#1{\lr[{#1}]} %square bracket
\def\brc{\set} %curly bracket, braces
\def\cbr{\set}
\def\emp{\cdot,\cdot} %empty parameters
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}

\def\rbig#1{\big(#1\big)}
\def\rBig#1{\Big(#1\Big)}
\def\rbigg#1{\bigg(#1\bigg)}
\def\rBigg#1{\Bigg(#1\Bigg)}
\def\sth#1#2{\lr.{#1}|_{#2}}
\def\sbig#1{\big[#1\big]}
\def\sBig#1{\Big[#1\Big]}
\def\sbigg#1{\bigg[#1\bigg]}


\def\nspc#1{\hspace{-2.5pt}#1\hspace{-2.5pt}}%neg. space
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\nspc{(#1)})} %formal Laurent series ((#1))
\def\cps#1{\{#1\}} %convergent power series
\def\cls#1{(\nspc{\cps{#1}})} %convergent Laurent series
\def\angg#1{\ang{\nspc{\ang{#1}}}}
%\def\nop#1{\left.\col\nspc{#1}\col\right.}%normally ordered product
%\def\nop#1{\,{\col#1\,\col}\,}   %% normally ordered
\def\scol#1{\scalebox{#1}{\ensuremath\col}} %scale column
\def\scalemacro#1{\mathchoice{#1{1.2}}{#1{1.2}}{#1{1}}{#1{1}}}
\def\nop#1{\,\scalemacro\scol#1\scalemacro\scol\,}


\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smatr#1{\begin{smallmatrix}#1\end{smallmatrix}}
\def\smat#1{\rbr{\smatr{#1}}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
%\def\eq#1{\begin{equation}#1\end{equation}} %used for equalizers
\RequirePackage{mathtools}
\def\ctr{\overbracket[.5pt][2pt]} %contraction, requires mathtools


%%%% Diff
\def\brake{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\imp$(#2).}}
\def\ddir#1#2{\noindent\textbf{(#1)$\iff$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
%\def\ie{i.e.,\,} %id est
%\def\eg{e.g.\@\xspace} %exempli gratia
%\def\cf{cf.\@\xspace} %confer
\def\ie{i.e.\@\xspace} %id est
\def\eg{e.g.\ } %exempli gratia
\def\cf{cf.\ } %confer
\def\lci{l.c.i.\@\xspace}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
%\def\wlog{without loss of generality\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\fae{following are equivalent\xspace}
\def\tfae{the \fae}
\def\nbd{neighborhood\xspace}
\def\fdd{finite-dimensional\xspace} % \fd used for \mathfrak{d}
\def\ifft{if and only if\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}
\def\eprint#1{\href{https://arxiv.org/abs/#1}{\ttfamily#1}}

%%%% Colons
\mathchardef\col\mathcode`:
\mathchardef\latexequal\mathcode`=
\def\ordinarycolon{\col} %used in \coloneqq and \vcentcolon

\def\colon{\nobreak \mskip 2mu\mathpunct {}\nonscript \mkern -\thinmuskip {\col}\mskip 6muplus1mu\relax}

\RequirePackage{mathtools} %for \coloneqq

{\makeatletter
  \catcode`:=\active
  \gdef:{\@ifnextchar={\coloneqq\@gobble}{\colon}}
  \catcode`==\active
  \gdef={\@ifnextchar:{\eqqcolon\@gobble}{\latexequal}}
}
\AtBeginDocument{\mathcode`:="8000\mathcode`=="8000}


%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
  \ifstrempty{#1}{}{\ifmmode#1\else\emph{#1}\fi}%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}


%%% Notes
\ifx\note\undefined
\RequirePackage[framemethod=TikZ]{mdframed}
\mdfsetup{backgroundcolor=brown!10, linewidth=0,
  skipabove=5pt, roundcorner=5pt}

\theoremstyle{definition}
\newmdtheoremenv[innertopmargin=-2pt]{note}{Note}
\newenvironment{notes}{\begin{note}}{\end{note}}

\newenvironment{comm}[1][brown!10]
  {\begin{mdframed}[backgroundcolor=#1]}{\end{mdframed}}
\newcommand\memo[2][brown!10]{
  \begin{mdframed}[backgroundcolor=#1]#2\end{mdframed}}
\def\red#1{\textcolor{red}{#1}}
\fi

%custom number side in equations, manual number: \tag{name}
\makeatletter
\def\leqnomode{\tagsleft@true\let\veqno\@@leqno}
\def\reqnomode{\tagsleft@false\let\veqno\@@eqno}
\makeatother


%custom theorem, can be used to list axioms (with labels)
\ifx\customthm\undefined
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\fi

% short names for theorems
\def\shortThm{
\envalias{thm}{theorem}
\envalias{thr}{theorem}
\envalias{dfn}{definition}
\envalias{lmm}{lemma}
\envalias{crl}{corollary}
\envalias{prp}{proposition}
}

\makeatother

%%%% Tikz %%%%
%\long\def\command#1{\providecommand{#1}{}\renewcommand{#1}}
\def\vcenterx#1{\ensuremath{\vcenter{\hbox{#1}}}}
\newcommand\btikz[2][]{\vcenterx{\tikz[#1]{#2}}} %base line
\newcommand\ctikz[2][]{\begin{center}\tikz[#1]{#2}\end{center}}

\def\eq#1{\begin{equation}#1\end{equation}}
%\def\i{^{-1}}

%%% Redefine \newcommand
%\makeatletter
%\let\oldcomm\newcommand
%\def\newcommand{\@ifstar{\oldcomm}{\newcomm}}
%\def\newcomm#1{
%  \@ifundefined{\expandafter\@gobble\string#1}
%    {\oldcomm{#1}}{\renewcommand{#1}}%
%}


